A computationally efficient robust model predictive control framework for uncertain nonlinear systems -- extended version

In this paper, we present a nonlinear robust model predictive control (MPC) framework for general (state and input dependent) disturbances. This approach uses an online constructed tube in order to tighten the nominal (state and input) constraints. To facilitate an efficient online implementation, the shape of the tube is based on an offline computed incremental Lyapunov function with a corresponding (nonlinear) incrementally stabilizing feedback. Crucially, the online optimization only implicitly includes these nonlinear functions in terms of scalar bounds, which enables an efficient implementation. Furthermore, to account for an efficient evaluation of the worst case disturbance, a simple function is constructed offline that upper bounds the possible disturbance realizations in a neighbourhood of a given point of the open-loop trajectory. The resulting MPC scheme ensures robust constraint satisfaction and practical asymptotic stability with a moderate increase in the online computational demand compared to a nominal MPC. We demonstrate the applicability of the proposed framework in comparison to state of the art robust MPC approaches with a nonlinear benchmark example. This paper is an extended version of [1], and contains further details and additional considers: continuous-time systems (App. A), more general nonlinear constraints (App. B) and special cases (Sec. IV).

==> old/Robust_Additive.tex <==
%!TEX root = ./Robust_Nonlin.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\subsection{Additive Disturbance and offline constraint tightening}
%
\textbf{change order --> make initial explainations for general setup}

\textbf{A simple way to treat the uncertainty, is to consider a constant upper bound $\overline{w}$\\Explain why conservative, say most paper do exactly do, explain advantage: computations can be done offline}

Let us first consider the simpler case of a nonlinear system subject to additive disturbances, as follows
\begin{align}
\label{eq:sys_w_additive}
x(t+1)&=f(x(t),u(t)) + w(t),\\
\|w(t)\|& \leq \bar{w}=\sup_{(x,u)\in\mathcal{Z}}\hat{w}(x,u).
\end{align}
where $w(t) \in \mathbb{R}^n$. 
\textbf{Redefine $\overline{w}$ as impact on incremental Lyapunov function $V_{\delta}$}
For this setup, we show that we can compute a suitable constraint tightening offline, that ensures robust closed-loop properties. 
A preliminary\footnote{
Compared to~\cite{JK_robust}, the following constraint tightening is less conservative, a more general stage cost is considered and terminal ingredients are included. 
} version of the resulting robust MPC has been presented in~\cite{JK_robust}. 
This formulation allows us to consider the case of state and input dependent disturbances as an extension. 
Let us define the scalars
\begin{align}
\label{eq:bar_w_N}
\bar{w}_N &= \rho^N\bar{w}\sqrt{c_{\delta,u}/c_{\delta,l}},\\
\label{eq:bar_c_j}
\bar{c}_{j} &= c_j\bar{w}\sqrt{c_{\delta,u}}, \quad j = 1, \dots, p.
\end{align}
The following assumption captures the sufficient properties of the terminal set in the case of additive disturbances, compare~\cite{chen1998quasi}.
\begin{assumption}
\label{ass:term} 
There exist a terminal controller $k_f:\mathbb{R}^n\rightarrow\mathbb{R}^m$, a terminal cost function $V_f:\mathbb{R}^n\rightarrow \mathbb{R}_{\geq 0}$, and a terminal set $\mathcal{X}_f=\{x\in\mathbb{R}^n|~V_f(x)\leq \alpha\}$, such that the following properties hold for any $x\in\mathcal{X}_f$ and any $w:$  $\|w\|\leq\bar{w}_N$ 
\begin{subequations}
\label{eq:term_dist}
\begin{align}
\label{eq:term_dist_dec}
V_f(x^+)\leq& V_f(x)-l(x,k_f(x)),\\
\label{eq:term_dist_RPI}
V_f(x^++w)\leq& \alpha,\\
\label{eq:term_dist_con}
L_{j,x}x + L_{j,u}k_f(x)\leq& 1-\dfrac{1-\rho^N}{1-\rho}\bar{c}_{j}, \quad j = 1, \dots, p,
\end{align}
\end{subequations}
with $x^+=f(x,k_f(x))$.  
Furthermore, the terminal cost is continuous on $\mathcal{X}_f$, i.e., there exists a function $\alpha_f\in\mathcal{K}$ such that 
\begin{align}
\label{eq:term_contin}
V_f(z)\leq V_f(x)+\alpha_f(\|x-z\|),
\end{align}
holds for all $x,~z\in\mathcal{X}_f$
\end{assumption}
Compared to the nominal Assumption on the terminal ingredients, the terminal set needs to be chosen smaller due to the constraint tightening, compare~\eqref{eq:term_dist_con}. 
In addition, robust positive invariance of the terminal set needs to be verified~\eqref{eq:term_dist_RPI}, which can be done based on~\eqref{eq:term_contin} and~\eqref{eq:term_dist_dec}. 
A simple formula for $\overline{w}$ in case of quadratically bounded cost functions $l,~V_f$ can be found in~\cite[Prop.~4]{JK_QINF}. 
Similar to nominal MPC, the theoretical properties can also be guaranteed without terminal ingredients under suitable assumptions, compare~\cite{grune2017nonlinear,JK_robust}.  

The open-loop cost of a state and input sequence $x(\cdot|t)\in \mathbb{R}^{n\times N+1},~u(\cdot|t)\in\mathbb{R}^{m\times N}$ is defined as
\begin{align}
\label{eq:J_N}
&J_N(x(\cdot | t),u(\cdot|t))=\sum_{k=0}^{N-1}l(x(k|t),u(k|t))+V_f(x(N|t)). 
\end{align}
The robust MPC scheme for additive disturbances is characterized by the solution of the following optimization problem
\begin{subequations}
\label{eq:MPC}
\begin{align}
V_N(x(t))&=\min_{u(\cdot|t)} J_N(x(\cdot | t),u(\cdot|t))\\
\text{s.t. }
&x(0|t)=x(t), \\
& x(k+1|t)=f(x(k|t),u(k|t)),\\
\label{eq:MPC_con}
&L_{j,x}x(k|t) + L_{j,u}u(k|t)\leq 1-\dfrac{1-\rho^k}{1-\rho}\bar{c}_{j},\\
\label{eq:MPC_term}
&x(N|t)\in\mathcal{X}_f,\\
& k=0,\dots, N-1,\quad j=1,\dots p.\nonumber
\end{align}
\end{subequations}
Compared to a nominal MPC, the only difference is that the tightened constraints~\eqref{eq:MPC_con} are considered along the prediction horizon. 
The solution of \eqref{eq:MPC} is the value function $V_N$, and optimal state and input trajectories $(x^*(\cdot|t)$, $u^*(\cdot|t))$ that satisfy the tightened constraints \eqref{eq:MPC_con}, the terminal constraint \eqref{eq:MPC_term} and minimize the cost $J_N$ over the prediction horizon $N\in\mathbb{N}$.
The closed-loop system is given by
\begin{align}
\label{eq:close}
x(t+1)=f(x(t),u(t))+w(t),\quad u(t)=u^*(0|t).
\end{align}
The following theorem establishes the closed-loop properties. 
\begin{theorem}
\label{thm:robust_simple}
Let Assumptions~\ref{ass:stage_cost}, \ref{ass:contract} and \ref{ass:term} hold. 
Assume that the disturbance bound $\bar{w}$ satisfies
\begin{align}
\label{eq:bound_bar_w}
\bar{w}\leq \sqrt{\delta_{\text{loc}}/c_{\delta,u}}.
\end{align}
Assume that~\eqref{eq:MPC} is feasible at $t=0$, then~\eqref{eq:MPC} is recursively feasible and the origin is practically asymptotically stable for the resulting closed-loop system~\eqref{eq:close}.
\end{theorem}
\begin{proof}
The proof is similar to~\cite{JK_robust}. 
The basic idea is to use the control law $\kappa$ from Assumption~\ref{ass:contract} to stabilize the previous optimal solution to~\eqref{eq:MPC} and thus bound the cost increase and ensure robust recursive feasibility. \\
\textbf{Part I:} Candidate input sequence and satisfaction of~\eqref{eq:MPC_con}:\\
For convenience, define
\begin{align*}
u^*(N|t)=k_f(x^*(N|t)), ~ x^*(N+1|t)=&f(x^*(N|t),u^*(N|t)),\\
u^*(N+1|t)=&k_f(x^*(N+1|t)).
\end{align*}
Consider the sequence
\begin{align}
\label{eq:robust_candidate}
 x(0|t+1)=&x(t+1)=x^*(1|t)+w(t),\\
u(k|t+1)=&\kappa(x(k|t+1),x^*(k+1|t),u^*(k+1|t)),\nonumber\\
x(k+1|t+1)=&f(x(k|t+1),u(k|t+1)),~ k=0,\dots,N. \nonumber
\end{align}
%
Due to continuity of $V_{\delta}$, \eqref{eq:bound} and \eqref{eq:bound_bar_w}, we have 
\begin{align*}
V_{\delta}(x(t+1),x^*(1|t), u^*(1|t))
\stackrel{\eqref{eq:bound}}\leq c_{\delta,u}\bar{w}^2 \stackrel{\eqref{eq:bound_bar_w}}\leq \delta_{loc}.
\end{align*}
Using the contractivity~\eqref{eq:contract} recursively, we get
\begin{align}
\label{eq:prop_robust_1}
V_{\delta}(x(k|t+1),x^*(k+1|t),u^*(k+1|t))\leq \rho^{2k} c_{\delta,u} \bar{w}^2\leq \delta_{loc}
\end{align}
for all $k=0,\dots,N$. 
Using \eqref{eq:lipschitz}, \eqref{eq:bar_c_j}, \eqref{eq:MPC_con} and \eqref{eq:prop_robust_1}, this implies that for all $k=0,\dots,N-2$ we have
\begin{align*}
&L_{j,x}x(k|t+1)+L_{j,u}u(k|t+1)\\
\stackrel{\eqref{eq:lipschitz}}{\leq}& L_{j,x}x^*(k+1|t) + L_{j,u}u^*(k+1|t)\\
&+c_j\sqrt{V_{\delta}(x(k|t+1),x^*(k+1|t),u^*(k+1|t))}\\
\stackrel{\eqref{eq:MPC_con}\eqref{eq:prop_robust_1}}{\leq} &1-\dfrac{1-\rho^{k+1}}{1-\rho}\bar{c}_{j}+c_j\rho^{k} \sqrt{c_{\delta,u}} \bar{w}\stackrel{\eqref{eq:bar_c_j}}=1-\dfrac{1-\rho^k}{1-\rho}\bar{c}_{j}.
\end{align*}
For $k=N-1$, condition~\eqref{eq:term_dist_con} in combination with $x(N|t)\in\mathcal{X}_f$ ensures the same property. \\
\textbf{Part II:} Terminal constraint~\eqref{eq:MPC_term}: 
Note that \eqref{eq:bound} and~\eqref{eq:prop_robust_1} imply
\begin{align*}
&\|x^*(N+1|t)-x(N|t+1)\| \\
\stackrel{\eqref{eq:bound}}{\leq}&\sqrt{\frac{1}{c_{\delta,l}} V_{\delta}(x(N|t+1),x^*(N+1|t),u^*(N+1|t))}\\
 \stackrel{\eqref{eq:prop_robust_1}}{\leq}& \sqrt{\frac{c_{\delta,u}}{c_{\delta,l}}}\bar{w}\rho^N \stackrel{\eqref{eq:bar_w_N}}= \bar{w}_N,
\end{align*} 
 and thus $x(N|t+1)\in\mathcal{X}_f$ due to Ass. \ref{ass:term} and~\eqref{eq:term_dist_RPI}. \\
\textbf{Part III:} Show practical stability: 
Given Proposition \ref{prop:contract} we have:
\begin{align*}
&l(x(k|t+1),u(k|t+1))-l(x^*(k+1|t),u^*(k+1|t))\\
\leq& \alpha_u(V(x(k|t+1), x^*(k+1|t), u^*(k+1|t))\\
\leq& \alpha_u(\rho^{2k} V(x(0|t+1), x^*(1|t), u^*(1|t)) \\
\leq & \alpha_u (c_{\delta,u}\overline{w}^2).
\end{align*}
Similar to~\cite[Prop.~5]{JK_robust}, feasibility of the candidate solution, summing up the stage cost $l$ and using the bound~\eqref{eq:term_contin}, yields
\begin{align*}
&V_N(x(t+1))\leq J_N(x(t+1),u(\cdot|t+1))\\
\leq& V_N(x(t))-l(x(t),u(t))+\alpha_f(\bar{w}_N) + N\alpha_u(c_{\delta,u}\overline{w}^2).
\end{align*}
Thus, the closed-loop system is practically asymptotically stable with the Lyapunov function $V_N$, compare~\cite[Prop.~11]{rawlings2012postface}.
\end{proof}
This result certifies that the constraint tightening~\eqref{eq:MPC_con} ensures that the desirable properties of MPC (recursive feasibility, constraint satisfaction, stability) are preserved despite additive disturbances. 
In case of quadratic stage cost better stability guarantees can be derived which do not scale with the prediction horizon $N$~\cite[Prop.~5,~Thm.~8]{JK_robust}, which is however not the focus of this paper. 
This result can be directly extended to consider time-varying bounds $\hat{w}$ on the additive disturbance with a time-varying constraint tightening, assuming this bound is known in advance. 
In the next section we show that it can also be extended to the less trivial and more challenging case of state and input dependent disturbances/uncertainty, where the future disturbance depends on the chosen control action. 



\end{comment}





